Improving Database Performance by Application-side Transaction Merging

This paper explores a new opportunity to improve the performance of transaction processing at the application side by merging structurely similar statements or transactions. Concretely, we re-write transactions to 1) merge similar statements using specific SQL semantics; 2) eliminate redundant reads; and 3) merge contending statements across transactions by pre-computing their aggregated effect. Following this idea, we present the design of TransactionMerger, a middleware to collect and merge transactions across different clients. We further present a static analysis tool to identify the merging opportunity without violating isolation as well as our experience of re-writing transactions in TPC-C and Spree, a popular real-world application. Our evaluation shows that such transaction merging can improve TPC-C throughput by up to 2.65X and Spree throughput by 3.52X.

==> algo.tex <==
\begin{algorithm}
\caption{Part 1: Offline Conflict-aware Grouping Statements}
\begin{algorithmic}[1]
\Statex \textbf{Input:} $T_{type}=(S_1, S_2, \dots, S_n)$, the statement template of a transaction type.
\Statex \textbf{Input:} $D_{intra}$, a set of all intra-transaction dependencies ($S_i \rightarrow S_j$).
\Statex \textbf{Output:} $P_{static}$, the Static Execution Plan, an ordered list of statement type groups.
\State $P_{static} \leftarrow []$, $D_{pairs} \leftarrow \{(S_i, S_j) | S_i \rightarrow S_j \in D_{intra}\}$, $i \leftarrow 1$

\While{$i \le n$}
    \State $S_{curr} \leftarrow S_i$
    \Statex \textbf{// Check if $S_{curr}$ is the source ($S_a \rightarrow S_{curr}$) of any dependency}
    \State $IsDependent \leftarrow \exists (S_a, S_b) \in D_{pairs}$ such that $\text{Index}(S_a) = i$

    \If{$IsDependent$}
        \Statex \textbf{// Start of a dependency group: Find the maximal span $k_{start}$ to $k_{end}$}
        \State $k_{start} \leftarrow i$, $k_{end} \leftarrow i$
        \State $SpanChanged \leftarrow \mathbf{true}$
    
        \While{$SpanChanged$}
            \State $SpanChanged \leftarrow \mathbf{false}$
            \State $NewEnd \leftarrow k_{end}$
        
            \Statex \textbf{// Check only dependencies where the source is within the current span $[k_{start}, k_{end}]$}
            \For{each $(S_a, S_b) \in D_{pairs}$}
                \State $idx_a \leftarrow \text{Index}(S_a)$, $idx_b \leftarrow \text{Index}(S_b)$
            
                \If{$k_{start} \le idx_a \le k_{end}$}
                    \Statex \textbf{// Dependency starts in the span; extend $NewEnd$ to include $S_b$}
                    \State $NewEnd \leftarrow \max(NewEnd, idx_b)$
                \EndIf
            \EndFor
        
            \If{$NewEnd > k_{end}$}
                \State $k_{end} \leftarrow NewEnd$
                \State $SpanChanged \leftarrow \mathbf{true}$
            \EndIf
        \EndWhile
    
        \State $G_{dependent} \leftarrow []$
        \Statex \textbf{// Group includes all statements in the contiguous block [$k_{start}, k_{end}$]}
        \For{$j$ from $k_{start}$ to $k_{end}$}
            \State $G_{dependent}$.append($S_j$)
        \EndFor
    
        \State $P_{static}$.append($G_{dependent}$)
        \State $i \leftarrow k_{end} + 1$
    
    \Else
        \Statex \textbf{// Statement without dependency forms a single-statement group.}
        \State $G_{single} \leftarrow \{S_{curr}\}$
        \State $P_{static}$.append($G_{single}$)
        \State $i \leftarrow i + 1$
    \EndIf
\EndWhile
\State \Return $P_{static}$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Part 2: Online Batch Execution}
\begin{algorithmic}[1]
\Statex \textbf{Input:} $\mathcal{T} = {T_1, T_2, \ldots, T_k}$: A batch of $k$ real transaction instances.
\Statex \textbf{Input:} $P_{static}$: The Static Execution Plan generated in Part 1.
\Statex \textbf{Output:} $L_{final}$: A final list of mergable batches to be executed.

\State $L_{final} \leftarrow []$
\For{each group $g=(S_a, S_b, \ldots)$ in $P_{static}$}
    \Statex \textbf{// Populate initial group from k transaction instances.}
    \State $B_{pending} \leftarrow []$
    \For{$i \gets 1$ to $k$}
        \State $instance \leftarrow (s_{(i,a)}, s_{(i,b)},\ldots)$ in $T_i$
        \State $instance.keys \leftarrow$ getRuntimeKeys($instance$)
        \State $B_{pending}$.add($instance$)
    \EndFor
    \Statex \textbf{// Refine the group by eliminating conflicting instances.}
    \While{$B_{pending}$ is not empty}
        \State $Batches_{current} \gets [[],[],\ldots]$: one list for each statement in $g$
        \State $conflict\_keys \gets \{\}$
        \State $B_{next} \gets []$
        \For{each $instance$ in $B_{pending}$}
            \If{$instance.keys \cap conflict\_keys = \emptyset$}
                \State// No conflict, add to current batch
                \For{each statement $s$ in $g$}
                    \State $Batches_{current}[s]$.add($instance.s$)
                \EndFor
                \State $conflict\_keys$.add($instance.keys$)
            \Else
                \State // Conflict, defer to next round.
                \State $B_{next}$.add($instance$)
            \EndIf
        \EndFor

        \For{each $batch$ in $Batches_{current}$}
            \State $L_{final}$.add($batch$)
        \EndFor
        \State $B_{pending} \gets B_{next}$
    \EndWhile
    \Statex \textbf{// Fully process this group, continue to the next.}
\EndFor
\State \Return $L_{final}$
\end{algorithmic}
\end{algorithm}

==> figures/alltxn.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\columnwidth]{evaluation/plot/alltxn_histogram.eps}
    \caption{Throughput of TPC-C five transactions of different warehouses under original, NoRPC merging and RPC merging settings.}
%    \vspace{-.1in}
    \label{fig:tpcc-alltxn}
\end{figure}


==> figures/micro.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{evaluation/plot/micro_select.pdf}
        \caption{Select}
        \label{fig:micro-select}
    \end{subfigure}
    %\hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{evaluation/plot/micro_update.pdf}
        \caption{Update}
        \label{fig:micro-update}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{evaluation/plot/micro_insert.pdf}
        \caption{Insert}
        \label{fig:micro-insert}
    \end{subfigure}
    %\hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{evaluation/plot/micro_delete.pdf}
        \caption{Delete}
        \label{fig:micro-delete}
    \end{subfigure}
       \caption{Throughput of Micro-benchmark}
       \label{fig:micro}
\end{figure*}

==> figures/neworder.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\columnwidth]{evaluation/plot/neworder_histogram.eps}
    \caption{Throughput of TPC-C NewOrder transaction of different warehouses under original, NoRPC merging and RPC merging settings.}
%    \vspace{-.1in}
    \label{fig:tpcc-neworder}
\end{figure}

